Grassmann Stein Variational Gradient Descent

Stein variational gradient descent (SVGD) is a deterministic particle inference algorithm that provides an efficient alternative to Markov chain Monte Carlo. However, SVGD has been found to suffer from variance underestimation when the dimensionality of the target distribution is high. Recent developments have advocated projecting both the score function and the data onto real lines to sidestep this issue, although this can severely overestimate the epistemic (model) uncertainty. In this work, we propose Grassmann Stein variational gradient descent (GSVGD) as an alternative approach, which permits projections onto arbitrary dimensional subspaces. Compared with other variants of SVGD that rely on dimensionality reduction, GSVGD updates the projectors simultaneously for the score function and the data, and the optimal projectors are determined through a coupled Grassmann-valued diffusion process which explores favourable subspaces. Both our theoretical and experimental results suggest that GSVGD enjoys efficient state-space exploration in high-dimensional problems that have an intrinsic low-dimensional structure.

==> SteinsGate (final)/sections/1_introduction.tex <==
Variational inference (VI) \citep{blei2017variational} is an optimisation-centric framework for approximating complex distributions that are intractable (only known up to a scale factor): given any target distribution $p(x)$, VI searches over a user-defined class of distributions $\mathcal{Q}$ for an optimal $q(x) \in \mathcal{Q}$ that is closest (in terms of a discrepancy or divergence) to $p(x)$. Extensively applied in the field of Bayesian inference, VI has the attraction of being scalable to big datasets, although it leads to biased estimation unless $\mathcal{Q}$ is broad enough to include the target distribution. This is in contrast to Markov chain Monte Carlo (MCMC) algorithms \citep{gilks1995markov}, which allows asymptotically exact sampling from the true target distribution, but does not scale well to big datasets and high dimensionality due to long mixing times \citep{levin2017markov}.

% \jef{What is the factor here O(..,)}\hz{it's the mixing time, albeit linear to the number of datapoints and dim  I SEE}
%(although scalable MCMC algorithms have been recently investigated. See \citep{welling2011bayesian}). 

The choice of $\mathcal{Q}$ in VI is crucial to guarantee a good approximation to $p(x)$ while retaining computational tractability. The classical mean-field approximation, which assumes that the distributions in $\mathcal{Q}$ have independent marginals, can be overly simplistic in many cases. To address this, a growing line of work in VI with Normalising Flows (NFs) \citep{rezende2015variational} seeks to construct an invertible map $T$ so that the pushforward distribution of $T(x)$, with $x\sim q$ and $q \in \mathcal{Q}$, will form a flexible approximation to $p$. 

Stein variational gradient descent (SVGD) \citep{Liu2016} was introduced as a particle-based variational inference method in which the map $T$ seeks to move a set of {particles} along a vector field which is chosen within a reproducing kernel Hilbert space (RKHS) to optimally transport towards the target $p(x)$.  Building on the kernel Stein discrepancy \citep{Liu2016}, the SVGD transport both drives the particles to the high-probability regions of $p(x)$ and enforces repulsion between the particles to prevent mode-collapse. It hence has the advantage of being ``particle-efficient'' in that a small number of particles can achieve good approximation of $p(x)$. Although this has made SVGD a popular tool in a range of applications including meta-learning \citep{yoon2018bayesian} and learning diversified mixture models \citep{wang2019nonlinear}, it is found that the marginal variance of the resulting particles scales inversely with the dimension, resulting in under-estimation of the variance. This was studied analytically in \cite{ba2022understanding}, in which the authors attributes this issue to \emph{(i)} an uneven scale of variance for the two terms in the SVGD update, and \emph{(ii)} a deterministic bias due to the dependence of the particle positions at each step.

% \ad{We  need to cite: \cite{ba2019towards} which carefully characterises the curse of dimensionality inherent in standard SVGD.}
% \xl{...can achieve decent approximations. Although this has made SVGD a popular tool in a range of applications from meta-learning \cite{yoon2018bayesian} to learning diversified mixture models \cite{wang2019nonlinear}, it is known that the marginal variance of the resulting particles scales inversely with the dimension, resulting in variance underestimation and model collapse. This \emph{curse of dimensionality} has been characterised in \cite{ba2019towards} to be caused by using estimates for the two terms that have variances of different scales and large bias introduced by the deterministic update.}

% To tackle this issue, message-passing Stein variational gradient descent (MP-SVGD) \cite{zhuo2018message} proposed a solution when $\pi(x)$ has a graphical model structure, although this will only apply to a limited selection of problems. Recently, slicing has been proposed for a number of problems to address high-dimensionality with sparsity \cite{rabin2011wasserstein,deshpande2019max}. In particular, the sliced kernel Stein discrepancy (SKSD) \cite{gong2021sliced, gong2021active} can been applied to SVGD by replacing the underlying kernel Stein discrepancy (KSD) with a one-dimensional projected version and this has been shown to resolve mode-collapse in many cases. Talk about pSVGD...

% \xl{This issue has been partially addressed in a limited selection of problems where $\pi$ is defined on \emph{known} Markov blankets \cite{wang2019stein,zhuo2018message}. For more generic settings, the idea of \emph{slicing} has been adopted where the kernel Stein discrepancy (KSD) in the derivation of SVGD is replaced with a one-dimensional version named \emph{maxSKSD} \cite{gong2021sliced}. This has been shown empirically to alleviate the mode-collapse issue of SVGD in toy Gaussian examples. Another work, called \emph{projected SVGD} (pSVGD) \cite{chen2020projected}, explored a similar idea where the particles are updated in adaptively constructed low-dimensional subspaces. This leads to a biased inference algorithm that requires expansive eigen-decomposition at each step.  }

% This issue has been partially addressed in a limited selection of problems where $p$ is defined on \emph{known} Markov blankets \cite{wang2019stein,zhuo2018message}. For more generic settings, \cite{chen2020projected} proposed the \emph{projected SVGD} (pSVGD), which updates the particles in adaptively constructed low-dimensional subspaces, leading to a biased inference algorithm that requires expensive eigen-decomposition at each step. In a more recent attempt, the idea of \emph{slicing} has been adopted, where the kernel Stein discrepancy (KSD) in the derivation of SVGD is replaced with a one-dimensional version named \emph{maxSKSD} \cite{gong2021sliced}. This has been shown empirically to alleviate the mode-collapse issue of SVGD in a range of examples. 

Recently, \cite{gong2021sliced} proposed a  \emph{sliced} version of kernel Stein discrepancy (KSD) analogous to other sliced discrepancies \citep{kolouri2019generalized}, and an associated \emph{sliced SVGD} (S-SVGD). This variant of SVGD decomposes the kernel-based dynamics along a sequence of 1-dimensional projections, called \emph{slices}.  Empirical results \cite[Appendix J.5, Table 5]{gong2021sliced} showed that the S-SVGD dynamic can mitigate the variance under-estimation issue of SVGD in high dimensions. However, S-SVGD is constrained to 1-dimensional projection, and only seeks the optimal slices for the data but keeps the slices for the score function deterministic. As we demonstrate in this paper, these can lead to inflated variance of the S-SVGD estimation. 
% On the contrary, SVGD will underestimate the uncertainty.


In this work, we introduce a unified approach where a non-uniform probability distribution over the projectors for \emph{both the score function and the data} are adaptively updated to emphasise directions in which there is largest discrepancy. This is achieved by introducing a stochastic diffusion process taking values in the Grassmann manifold \citep{bendokat2020grassmann} which evolves along with SVGD particles. By tuning the diffusion process parameters we can adjust the trade-off between exploration and exploitation of suitable projections. In addition, using projections onto higher dimensional spaces allows us to take into account the correlations/interactions between components and thus producing more accurate uncertainty estimates.

% \ad{TODO: Update the story.  Broadly speaking, the introduction of slicing into a discrepancy takes one of two forms: the \emph{average case sliced discrepancy } where we introduce a probability measure over the space of projectors and compute the average projected discrepancy, or the \emph{worst case sliced discrepancy} where one considers the maximum projected discrepancy over all projectors. Both approaches offer distinct advantages and present a trade-off between exploration and computational efficiency.  In this work we introduce a unified approach where a non-uniform probability distrbution over the slices is adaptively updated to emphasise directions in which there is largest discrepancy.  This is achieved by introducing a stochastic diffusion process taking values in the Grassmann manifold which evolves along with SVGD particles.  By tuning the diffusion process parameters we can adjust the trade-off between exploration and exploitation of suitable slice directions.} 

% \textbf{Our contributions:} Motivated by S-SVGD, we derive an alternative SVGD algorithm that also uses the idea of low-dimensional projections, which we call Grassmann SVGD (GSVGD), by projecting onto $m\geq1$ dimensions using the Grassmann manifold. By using a coupled Grassmann-valued diffusion process, we can learn the more efficiently explore the projections whilst performing SVGD. We show numerically that our method is competitive to SVGD and S-SVGD on high-dimensional synthetic and benchmark problems.
\textbf{Contributions:} 
Motivated by S-SVGD, we propose a novel algorithm, Grassmann SVGD (GSVGD), which employs $m$-dimensional projectors (compared with the $1$-dimensional ones in S-SVGD) to evolve the particles towards the target distribution and to mitigate variance under-estimation. We show numerically that our method is competitive to SVGD and S-SVGD on high-dimensional synthetic and benchmark problems while more accurately estimating the epistemic uncertainty.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/misc/summary.pdf}
    \vspace{-0.3cm}
    \caption{A summary of different SVGD algorithms using no projections (SVGD), 1-dimensional projections (S-SVGD), and $m$-dimensional projections (GSVGD) with an arbitrary $1 \leq m \leq d$, where $d$ is the dimensionality of the problem. }
    \label{fig: summary}
\end{figure}

==> SteinsGate (final)/sections/2_background.tex <==
\paragraph{Stein Variational Gradient Descent:} Let $\calX = \bbR^{d}$ and $P$ be a probability measure over $\calX$ with smooth positive density $p$ which we can evaluate up to a normalisation constant. We are interested in approximating $P$ by transporting a known measure $Q$, defined over $\calX$ and with smooth density $q$, to $P$ via a sequence of maps that minimise a given loss. 

Choosing the loss to be the Kullback-Leibler (KL) divergence defined as $\text{KL}(Q,P) = \int_{\calX}q(x)\log(q(x)/p(x))dx$ allows us to minimise the discrepancy $\text{KL}(T_{\#}Q,P)$  over maps $T\colon\calX\rightarrow\calX$ where $T_{\#}Q$ is the pushforward of $Q$ with respect to $T$. In \citet{Liu2016SVGD}, the authors choose a specific parametrisation $T(x) = x+\varepsilon\phi(x)$ where $\phi$ lies within the unit ball $\mathcal{B}_k^d:=\{\phi\in\mathcal{H}_k^d: ||\phi||_{\mathcal{H}_k^d}\leq 1\}$ of the Cartesian product $\mathcal{H}_k^d:=\bigtimes_{i=1}^d \mathcal{H}_k$ of the RKHS $\mathcal{H}_k$ associated with kernel $k:\mathcal{X}\times\mathcal{X}\rightarrow\mathbb{R}$. The crucial observation of \citet{Liu2016SVGD} is that the maximal rate of decay of this discrepancy with respect to $\epsilon$ is the kernel Stein discrepancy (KSD) \citep{Chwialkowski16,Liu2016} given by
\begin{talign}
    \text{KSD}(Q,P) 
    &= \sup_{\phi\in\mathcal{B}_k^d} \mathbb{E}_Q[\calA_{p}\phi(x)],\label{eq:KSD_def}
\end{talign}
where $x\sim Q$,  $s_{p}(x) = \nabla_{x}\log p(x)$ is the \emph{score function} and $\mathcal{A}_{p} \phi(x) = s_{p}(x)^\intercal\phi(x) + \nabla \cdot \phi(x)$ is the \textit{Stein operator} associated to $P$. The key advantage of KSD is that it quantifies the difference between two measures $P$ and $Q$ where only the score function of $P$ is available, which is the typical situation in Bayesian inference for complex models.  The supremum in \eqref{eq:KSD_def} is attained by the function $\phi^{*}(\cdot) 
\coloneqq \mathbb{E}_{Q}[\mathcal{A}_p k(\cdot,x)] =\mathbb{E}_Q[k(\cdot, x)s_{p}(x) +   \nabla_{x} k(\cdot, x)]$, which leads to the remarkable result \citep[Theorem 3.3]{Liu2016SVGD} $\nabla_\phi \text{KL}(T_{\#}Q,P)|_{\phi=0} = -\phi^{*}(x)$ where $\nabla_{\phi}$ is the functional derivative and $T(x)$ is the map parameterised as above. This suggests that $\phi^{*}$ is, according to KL divergence, the best choice of function to use in $T$ to map $Q$ to $P$. 

The expression for the optimal $\phi^*$ forms the basis of the SVGD algorithm.  Particles $X^t = (x_1^t,\ldots, x_N^t)$ at step $t$, are evolved using the following update rule
\begin{talign}
 \label{eq:svgd_vanilla}
    x_i^{t+1} 
    &= x_i^t + \epsilon  \widehat{\phi}^\ast(x_i^t),
\end{talign}
for $i=1,\ldots, N$ and $t=0, 1,2,\ldots$, where \begin{talign}
    \label{eq: svgd_vanilla update}
    \widehat{\phi}^*(\cdot) = \frac{1}{N}\sum_{j=1}^{N}\big[k(\cdot,  x_j^t)\nabla_{x^t_j}\log p(x_j^t) + \nabla_{x_j^t} k(\cdot, x_j^t)\big]
\end{talign} is an estimator of $\phi^*(\cdot)$ obtained by replacing $Q$  with  $\frac{1}{N}\sum_{i=1}^N \delta_{x_i^t}$. Intuitively, \eqref{eq:svgd_vanilla} is an Euler discretisation with step-size $\epsilon$ of the following system of ODEs
\begin{talign*}
    \frac{d x_i}{dt}(t) 
    &= \frac{1}{N}\sum_{j=1}^{N}\big[k(x_i(t),  x_j(t))\nabla_{x_j(t)}\log p(x_j(t)) \\ 
    &\quad + \nabla_{x_j(t)} k(x_i(t), x_j(t))\big], \quad i=1,\ldots,N,
\end{talign*}
for particle positions $x_1(t),\ldots, x_N(t)$.


\paragraph{Tackling the Curse of Dimensionality:}
The SVGD algorithm has shown to be asymptotically exact, in the sense that in the limit of infinite particles and vanishing step-size the particles will converge to the target density \citep{lu2019scaling}.  However, in  the finite particle regime,  SVGD may fail to adequately explore the state-space, exhibiting mode collapse and variance under-estimation, particularly in high dimensions \citep{Liu2016,zhuo2018message,gong2021sliced}.

The deterioration in performance in high-dimensions can be understood from the update rule defined in \eqref{eq: svgd_vanilla update}. The RHS consists of two terms: a kernel-averaged score function $\frac{1}{N}\sum_j k(\cdot, x_j^t)\nabla\log p(x_j^t)$ which attracts particles towards modes of the target density, and a repulsion term $\frac{1}{N}\sum_j \nabla k(\cdot, x_j^t)$ which encourages particle diversity by pushing nearby particles away from each other. As has been observed in \citet[Section 3.2]{Liu2016SVGD} and studied analytically in \cite[Section 3]{zhuo2018message}, the influence of the repulsion term drops dramatically with increasing dimension, effectively reducing SVGD to a gradient ascent method for $\log p$. As a result, the estimation of SVGD can suffer from a significant under-estimated variance for high-dimensional targets. 

Various developments have been proposed to mitigate this issue; we now discuss the most relevant to our work, the sliced approach of \citet{gong2021sliced}, and defer a review of the others to Section \ref{sec:related_work}. \citet{gong2021sliced} addressed this problem by projecting both the particles and the score function along one-dimensional directions, known as \emph{slices}, leading to the \emph{max sliced kernel Stein discrepancy} (maxSKSD). This approach hinges on the fact that measuring KSD along finitely many slices is sufficient to capture all geometric information of two distributions, as long as optimal slices are used. Given a user-defined orthonormal basis $O$ in $\bbR^d$, the \emph{maxSKSD} takes the form
\begin{align}
    &\text{maxSKSD}(Q,P) 
     =
     \sum_{r \in O} \sup_{g_{r}\in\mathbb{S}^{d-1}}\sup_{\phi \in \mathcal{B}_{k}} \bbE_Q[ s_p^r(x) \phi(x^{\intercal}g_{r}) \nonumber \\ 
     &\quad + r^\intercal g_{r} \nabla_{x^{\intercal}g_{r}} \phi(x^{\intercal}g_{r})],\label{eq:maxSKSD}\\
    &= \sum_{r \in O}\sup_{g_{r}\in\mathbb{S}^{d-1}}\sup_{\phi \in \mathcal{B}_{k_{r,g_{r}}}}\bbE_{Q}[s_{p}(x)^\intercal\phi(x) + \nabla\cdot\phi(x)]\label{eq:maxSKSD_mat}
\end{align}
where $s^r_p(x) \coloneqq s_p(x)^\intercal r$ is the score projected along a slicing direction $r$ and $\mathcal{B}_{k}$ is the unit ball of from RKHS $\calH_{k}$ for some kernel $k\colon\bbR\times\bbR\rightarrow\bbR$. The subscript $g_{r}$ is used to emphasise that for each $r$ a new optimal $g_{r}$ must be found. In \eqref{eq:maxSKSD_mat}, $\mathcal{B}_{k_{r,g_{r}}}$ is the unit ball of the RKHS corresponding to the matrix valued kernel $k_{r,g_{r}}(x,y) = rr^{\intercal}k(g_{r}^{\intercal}x,g_{r}^{\intercal}y)$. This can be seen from standard results regarding matrix valued kernels \citep[Chapter 6]{Paulsen2016} and this will be relevant to our later developments.

The idea of the maxSKSD approach is that the $r\in O$ will slice the score function of the target, and for each of those slices the input is sliced according to some other directions $g_{r}$. It is known that, under some standard regularity conditions, maxSKSD discriminates measures \citep[Corollary 3.1]{gong2021sliced}. Replacing KSD with maxSKSD in SVGD results in \emph{sliced-SVGD} (S-SVGD; \citet{gong2021sliced}). 

An issue with this procedure is that the basis $O$ is a user-defined choice and may result in inefficient performance. Additionally, restricting $g_{r}$ and $r$ to one dimension might not capture the underlying structure as effectively as higher dimensional projections. Our approach, described in Section \ref{sec:GSVGD}, will use projections onto subspaces that have dimension potentially greater than one. The framework of these subspace projections is described next. This framework also allows us to explore projections in the underlying geometry more efficiently by using Riemannian optimisation.


\paragraph{Grassmann Manifold}
Let $m \in \{ 1, 2, \ldots, d\}$. A crucial ingredient of our proposed method is the \emph{Grassmann manifold} of $m$-dimensional subspaces in $\bbR^d$ \citep{bendokat2020grassmann}, defined as
\begin{talign*}
    \textrm{Gr}(d, m) = \{ E \subseteq \bbR^d: \textrm{dim}(E) = m \}.
\end{talign*}
The intuition behind our proposed method is to define a KSD that seeks the worst possible discrepancy over all distinct subspaces of dimension $m$, where the worst-case subspace can be found with gradient-type optimisation on the Grassmann manifold. We briefly review the key ingredients of optimisation on the Grassmann manifold; a more detailed discussion is deferred to Appendix \ref{appendix: grassmann manifold}.

To make sense of optimisation on the Grassmann manifold, we first need to represent each subspace $E \in \textrm{Gr}(d, m)$ in memory. One way of doing so is by a projection operator that maps every $x \in \bbR^d$ to an element in the subspace. To this end, we define a \emph{projector} of rank $m$ to be a $d \times m$ matrix $A$ with orthonormal columns, i.e.\ $A^\intercal A = I_m$, where $I_{m}$ is the $m\times m$ identity matrix. It then follows that $A A^\intercal$ is a projection matrix since $(A A^\intercal)^2 = A A^\intercal$ and $(A A^\intercal)^\intercal = A A^\intercal$. Denote by $[A] = \{ A y: y \in \bbR^m \} \subset \bbR^d$ the image of $A$.

We represent each subspace $E \in \textrm{Gr}(d, m)$ by \emph{any} projector $A$ for which $[A] = E$. This is always possible since, for each projector $A$ the subspace $[A]$ is trivially an element of $\textrm{Gr}(d, m)$, and, conversely, for any $E \in \textrm{Gr}(d, m)$, we can construct a corresponding projector $A$ by column-wise appending the elements of any orthonormal basis of $E$. Such $A$ is unique up to an orthogonal transformation: for any projectors $A, B$, the subspaces $[A] = [B]$ if and only if $A = BC$ for some orthogonal matrix $C$ in $\bbR^{m \times m}$. As we will show in Section~ \ref{sec:GSD}, the proposed KSD does not depend on which projector is chosen so long as it corresponds to the same subspace $E$.

Given a representative $A$ of $[A] \in \textrm{Gr}(d, m)$, the \emph{tangent space} at $[A]$ is defined as $\mathcal{T}_{[A]}\text{Gr}(d,m)=\lbrace \Delta \in \mathbb{R}^{d \times m} : A^\intercal \Delta = 0 \rbrace$. We endow a Riemannian metric on $\mathcal{T}_{[A]}\text{Gr}(d,m)$ by restricting the standard matrix inner product $\langle \Delta, \tilde{\Delta} \rangle_0 = \Tr(\Delta^\intercal \tilde{\Delta})$ to elements $\Delta, \tilde{\Delta}$ in $\mathcal{T}_{[A]} \textrm{Gr}(d, m)$. It is then clear that $\Pi_A = I_d - A A^\intercal$ is a projection operator of $\bbR^{d \times m}$ onto $\mathcal{T}_{[A]} \textrm{Gr}(d, m)$: $\Pi_A G = (I_d - A A^\intercal) G \in \mathcal{T}_{[A]} \textrm{Gr}(d, m)$, for any $G \in \bbR^{d \times m}$ \cite[Proposition 3.53]{boumal2020introduction}.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/misc/rgd.pdf}
    \caption{An illustration of a gradient ascent step on the Grassmann manifold.}
    \label{fig: riemannian gradient descent}
\end{figure}

Let $\calF$ be a function defined on $\text{Gr}(d,m)$ that is smooth in a proper sense \cite[Section 3]{boumal2020introduction}. Given a base point $[A] \in \text{Gr}(d,m)$, maximising $\calF$ requires \emph{(i)} finding a vector field of steepest ascent of $\calF$ at $[A]$, and \emph{(ii)} moving from $[A]$ along that vector field without leaving the manifold. 

On the Grassmann manifold, the direction of steepest ascent is no longer represented by the standard (Euclidean) gradient $\nabla \calF([A])$. Instead, it is given by the \emph{Riemannian gradient} of $\calF$ at $[A]$, given by
\begin{talign*}
    \riemannGrad \calF = \Pi_A \nabla \calF([A]), 
\end{talign*}
where $[\nabla \calF([A])]_{ij} = \partial \calF([A]) / \partial A_{ij} $. That is, $\riemannGrad \calF$ is the projection of the Euclidean gradient $\nabla \calF([A])$ onto the tangent space at $[A]$. For \emph{(ii)}, one means of moving along a manifold in a given direction is by the \emph{exponential map} \cite[Section 10.2]{boumal2020introduction}. In our work, we use the \emph{polar retraction} \citep[Definition 3.41]{boumal2020introduction}, which is an accurate (second order) approximation of the exponential map that is amendable to computation, and is defined as
\begin{talign}
    \label{eq: polar retr}
    \textrm{R}_{[A]}(\Delta ) = [UV^\intercal] ,
\end{talign}
where $[A] \in \text{Gr}(d,m)$, and $A + \Delta = USV^\intercal$ is a thin Singular Value Decomposition (see e.g.\ \citet[Section 9.6]{boumal2020introduction}). 

To summarise, with a step-size $\delta > 0$, one step to maximise $\calF$ starting from a base point $[A]$ is given by
\begin{talign*}
    [A'] = \textrm{R}_{[A]}(\delta \riemannGrad \calF).
\end{talign*}
See~Fig.\ref{fig: riemannian gradient descent} for an illustration. This is a generalisation of the standard gradient ascent to the Grassmann manifold \cite[Section 4.3]{boumal2020introduction}.




==> SteinsGate (final)/sections/3_grassman_ksd.tex <==
The starting point of our proposed approach is to introduce a novel Stein discrepancy which incorporates dimension reduction features through the use of a projector. To this end, for a projector $A$ of rank $m$ we introduce a matrix-valued kernel $k_A$ arising from an embedding on $\mathbb{R}^d$ into a $m$-dimensional subspace where $m\leq d$
\begin{talign*}
    k_A(x,y) = A A^\intercal k(A^\intercal x, A^\intercal y),\quad  x,y\in \mathbb{R}^d,
\end{talign*}
where $k:\mathbb{R}^m\times \mathbb{R}^m\rightarrow \mathbb{R}$ is a scalar-valued positive definite radial kernel on $\mathbb{R}^m$. That is, 
$k(u,v)=\Psi(\lVert u-v\rVert_{2}), u,v\in \mathbb{R}^m$, where $\Psi\colon\bbR\rightarrow\bbR$ and $\lVert\cdot\rVert_{2}$ is the Euclidean $2$-norm. Before proceeding, since we shall be performing optimisation over $\text{Gr}(d,m)$, we must be sure that for any two projectors $A,B$ that are equivalent in Gr$(d,m)$ the kernels $k_{A},k_{B}$ are equal. The next lemma assures us of this (see Appendix~\ref{appendix: proof of lemma grassmann_kernel} for the proof).

% \begin{lemma}
% \label{lemma: grassmann_kernel}
% % The Grassman Kernel Stein Discrepancy $KSD_{A}(P,Q)$ is independent of the particular representer of the Grassmann element $[A]\in \mbox{Gr}(d,m)$.
% Let $A,B\in\emph{St}(d,m)$ with $A\sim B$ in $\emph{Gr}(d,m)$ then $k_{A} = k_{B}$.
% \end{lemma}
\begin{lemma}
\label{lemma: grassmann_kernel}
Let $A,B$ be projectors of rank $m$ with $[A] = [B]$, then $k_{A} = k_{B}$.
\end{lemma}
Safe in the knowledge that $k_{A}$ is well defined over $\text{Gr}(d,m)$, we may define an associated KSD, which reveals how this choice of $k_{A}$ induces a projection of the data and score function. 
\begin{align}
    \mbox{KSD}_{A}(Q,P) 
    &= \sup_{\phi\in\mathcal{B}_{k_{A}}}\bbE_{Q}[s_{p}(x)\cdot \phi(x) + \nabla\cdot\phi(x)]
    \label{eq:GKSD_vec}\\
    = \sup_{\phi\in\mathcal{B}_{k}^{m}}\bbE_{Q}&\big[(A^\intercal s_{p}(x))\cdot\phi(A^\intercal x)
     + \nabla\cdot \phi(A^\intercal x)\big] .
    \label{eq:KSD_A}
\end{align}
where $\mathcal{B}_{k_{A}}$ is the unit ball of the RKHS corresponding to $k_{A}$ and $\mathcal{B}_{k}^{m}$ is the unit ball of the $m$-times Cartesian product of $\calH_{k}$, the RKHS corresponding to $k$. Contrasting this to \eqref{eq:maxSKSD}, setting $m=1$ and $r,g_{r} = A$ results in \eqref{eq:KSD_A}. The $r^{\intercal}g_{r}$ term in \eqref{eq:maxSKSD} becomes $I_{m}$ in \eqref{eq:KSD_A} since $A$ has orthonormal columns. 


Analogous to the approach for KSD (see \citet{Liu2016}), we exploit the kernel trick to express $\text{KSD}_A$:
\begin{talign}
    &\text{KSD}_{A}(Q,P) \nonumber \\
    &=\mathbb{E}_{x, x'\sim Q}\left[ (A^\intercal s_{p}(x)) \cdot A^\intercal s_{p}(x')k(A^\intercal x,A^\intercal x')\right] \nonumber \\
    &\quad +2\mathbb{E}_{x, x' \sim Q}[ (A^\intercal s_{p}(x)) \cdot \nabla_{x_2}k(A^\intercal x,A^\intercal x')] \nonumber\\
    &\quad +\mathbb{E}_{x, x' \sim Q}[\Tr(\nabla_{x_1,x_2}k(A^\intercal x,A^\intercal x'))],\label{eq:KSD_double_integral}
\end{talign}
where $x, x'$ are i.i.d.\ random variables drawn from $Q$, $\nabla_{x_i} k(A^\intercal x, A^\intercal x')$ denotes the gradient of $k$ with respect to the $i$-th argument, $\nabla_{x_1,x_2}k$ is the matrix with $ij$-th entry $\partial^{2}k/\partial x_{i}\partial x_{j}$, and $\Tr(\cdot)$ denotes the trace.



It is clear that $\text{KSD}_{A}$ does not characterise probability measures for any fixed $A$.  For example if $P = \mathcal{N}(0,C)$ and $Q = \mathcal{N}(0, C')$ are distinct probability measures such that $A^\intercal C= A^\intercal C'$, then $\mbox{KSD}_{A}(Q,P) = 0$.  This motivates us to consider the worst-case discrepancy taken over all $m$-dimensional subspaces. We define the \emph{Grassmann Kernel Stein Discrepancy} (GKSD) as
\begin{talign}
\label{eq:GKSD}
    \text{GKSD}(Q,P) = \sup_{[A]\in \text{Gr}(d,m)} \text{KSD}_{A}(Q,P).
\end{talign}
The following theorem guarantees that GKSD is able to discriminate distinct distributions. The assumptions on $P,Q$ are standard \citep{gong2021sliced}.

\begin{theorem}\label{thm:KSD_separates}
Let $P,Q$ be Borel measures with continuously differentiable densities $p,q$ both supported on $\bbR^{d}$ with $\lim_{\|x\|_2\rightarrow \infty}q(x) = 0$ and suppose the kernel $k(u,v) = \Psi(\|u-v\|_2)$ is characteristic and bounded with continuous second order partial derivatives. Then the \emph{GKSD} \eqref{eq:GKSD} equals $0$ if and only if $p=q$.
\end{theorem}
\begin{remark}
A radial kernel $k(x,y) = \Psi(\|x-y\|_2)$ is characteristic if and only if it is integrally strictly positive definite \citep{sriperumbudur2011universality}. In particular, the assumptions of Theorem \ref{thm:KSD_separates} hold for Gaussian and Inverse Multiquadric kernels.
\end{remark}

Intuitively, projecting on higher dimensions for $s_p(x)$ will allow us to better account for the correlation between dimensions. With optimal projectors, correlations can be captured regardless of the projection dimension, since both GKSD and maxSKSD can discriminate distinct distributions. In practice, however, optimal projectors are not available, and hence projecting onto 1 dimension can lead to sub-optimal approximation due to weak correlation signals.



% To demonstrate the effectiveness of introducing a projection into the Stein discrepancy let us consider the situation where $P$ and $Q$ differ only along a finite dimensional subspace.  The following result demonstrates that GSVGD will recover the subspace along which the tw probabilities are differing.

% \begin{theorem}
% Let $P,Q$ be Borel measures with continuously differentiable positive densities $p,q$.  Given $B \in \mbox{St}(d,m)$ suppose that 
% $$
%     p(x) \propto r(Bx)\pi(x) \quad \mbox{ and }  q(x) \propto r'(Bx)\pi(x),
% $$
% for two positive densities $r$ and $r'$ on $\mathbb{R}^m$.   Then the maximum in \eqref{eq:GKSD_vec} is attained when $A \in [B]$ and
% $$
% \text{GSVGD}(P,Q) = \text{KSD}_k(A_\sharp P, A_\sharp Q),
% $$
% where $A_\sharp P$ and $A_\sharp Q$ denote the pushforwards of $P$ and $Q$ respectively, with respect to $A$.
% \end{theorem}
% \begin{proof}[\textbf{Proof (To be moved to appendix)}]

% We can write $\mbox{KSD}_A(Q,P)$ as 
% $$
% \mbox{KSD}_A(Q,P) = \int\int (A(s_p(x)-s_q(x))^\intercal (A(s_p(x)-s_q(x)) k(Ax,Ay)q(dx)q(dy),
% $$
% where $s_p(x)-s_q(x)  = B^\intercal \nabla \log l (Bx)$, for $l=r/r'$.  This yields
% $$
% \mbox{KSD}_A(Q,P)=\int\int (AB^\intercal \nabla l(Bx))^\intercal (AB^\intercal \nabla l(Bx)) k(Ax,Ay)q(dx)q(dy).
% $$
% Choosing $A=B$ we obtain
% \begin{align*}
% \mbox{KSD}_A(Q,P) = \mbox{KSD}_B(Q,P)&=\int\int ( \nabla l(Bx))^\intercal ( \nabla l(Bx)) k(Bx,By)Q(dx)Q(dy) \\ &= \int\int  \nabla l(x)^\intercal  \nabla l(x) k(x,y)B_\sharp Q(dx)B_\sharp Q(dy).
% \end{align*}
% We show that the right hand side is the maximum.  Another natural approach to defining a projected Stein discrepancy is by considering the KSD between the pushforward measures $A_\sharp P$ and $A_\sharp Q$ supported on $\mathbb{R}^m$, given by
% \begin{equation}
% \label{eq:pf_ksd}
%     \text{KSD}(A_\sharp Q,A_\sharp P) = \sup_{\substack {\phi \in \mathcal{H}_k \\ \lVert \phi\rVert_{H_k} \leq 1}}\mathbb{E}_{A_\sharp Q}\left[s_{A_\sharp p}(x)\cdot \phi(x) + \nabla\cdot \phi(x)\right],
% \end{equation}
% where 
% $$
%     s_{A_\sharp p}(y) = \nabla\log \int_{\lbrace{x \in \mathbb{R}^d  y=Ax}\rbrace} p(x)\,dx,
% $$is the score function associated with the push-forward measure $A_\sharp p$.   Simplifying \eqref{eq:pf_ksd} we obtain
% $$
%     \text{KSD}(A_\sharp Q,A_\sharp P) = \sup_{\substack {\phi \in \mathcal{H}_k \\ \lVert \phi\rVert_{H_k} \leq 1}}\mathbb{E}_{Q}\left[\nabla \log \int_{y\in \mbox{Ker}[A]}p(x+y)\,dy \cdot \phi(A x) + \nabla\cdot \phi(A x)\right]
% $$
% \end{proof}

==> SteinsGate (final)/sections/4_gsvgd.tex <==
Equipped with this new form of kernel discrepancy we can perform a variant of SVGD which we call \emph{Grassmann Stein Variational Gradient Descent} (GSVGD). More specifically, we seek to find 
\begin{talign}
    \label{eq:sliced_objective}
    \phi_{A}^* \in \arg\sup_{\phi \in \mathcal{B}_{k_A}} -\frac{d}{d\epsilon}\mbox{KL}(T_{\sharp}Q, P)\Big|_{\epsilon=0},
\end{talign}
where $T_\sharp = I + \epsilon \phi$, and $I$ is the identity map. The supremum on the RHS of \eqref{eq:sliced_objective} is attained by 
\begin{talign*}
    \phi_{A}^{*}(\cdot) = \bbE_{Q}[A A^\intercal s_{p}(x)k(A^\intercal x,A^\intercal \cdot) + A\nabla_{x_1}k(A^\intercal x,A^\intercal \cdot)],
\end{talign*}
for which it is clear that
\begin{talign*}
-\frac{d}{d\epsilon}\mbox{KL}(T^*_{\sharp}Q, P)\Big|_{\epsilon=0} = \mbox{KSD}_{A}(P,Q), \quad T^*_{\sharp} = I + \epsilon \phi^*_A.
\end{talign*}
To transport the particles efficiently, at every step, we seek to identify the subspace $[A] \in \text{Gr}(d,m)$ with the largest discrepancy between $P$ and $Q$, so that we select
\begin{talign}
    \label{eq:sliced_objective_A}
    [A^*] \in \arg\sup_{[A] \in \text{Gr}(d,m)} \mbox{KSD}_A(P,Q),
\end{talign}
for which $\mbox{KSD}_{A^*}=\mbox{GKSD}(P,Q)$. In practice, the objective (\ref{eq:sliced_objective_A}) can be (approximately) solved by searching for a critical point of $\mbox{KSD}_A(P, Q)$ at which its Riemannian gradient vanishes. This is justified by the following proposition, which states that, when the probability measures $P$ and $Q$ differ in some low-dimensional subspace $[A_0]$, then $[A_0]$ is indeed a solution sought by (\ref{eq:sliced_objective_A}).
\begin{proposition}
    Suppose the conditions in Theorem~\ref{thm:KSD_separates} hold for the kernel $k$ and measures $P, Q$ with associated densities $q, p$. Assume further that the kernel satisfies a smoothness condition Assumption \ref{assumption: smoothness of kernel} in Appendix~\ref{appendix: extra assumption on the kernel}, and that there exists $[A_0] \in \textrm{Gr}(d, m)$ such that $q, p$ admit the following decomposition
    \begin{talign}
        q(x) &\propto q^m(P_0 x) \xi(\Pi_{A_0} x) \label{eq: prop optimal projection, decomposition 1}\\ 
        p(x) &\propto p^m(P_0 x) \xi( \Pi_{A_0} x),
        \label{eq: prop optimal projection, decomposition 2}
    \end{talign}
    where $P_0 \coloneqq A_0 A_0^\intercal$, $\Pi_{A_0} = I_d - A_0 A_0^\intercal$ as before, and $p^m, q^m$ and $\xi$ are smooth, positive functions that are integrable on $\bbR^d$ (i.e.\ they are unnormalised densities). Then $\riemannGrad \mbox{KSD}_A(P,Q) |_{A = A_0} = 0$.
    \label{prop: optimal projection}
\end{proposition}

\begin{remark}
    The assumption on the decomposition (\ref{eq: prop optimal projection, decomposition 1}) and (\ref{eq: prop optimal projection, decomposition 2}) holds when the density $q$ agrees with the target $p$ except in the subspace $[A_0]$. An example is that $q$ is a prior, and $p$ is the posterior induced from $q$ and a likelihood function that depends on $x$ only through $A_0 x$. See Appendix \ref{appendix: lemma and proof of proposition 3} for more discussions and the proof.
\end{remark}

Sequentially solving the optimisation problems \eqref{eq:sliced_objective} and \eqref{eq:sliced_objective_A} every time-step yields a particle transport scheme which terminates if and only if the GKSD between the target distribution and the current particle distribution is zero, which implies $P=Q$ under the conditions of Theorem \ref{thm:KSD_separates}. 

Replacing $Q$ by an empirical distribution of particles $(x_1^0,\ldots, x_N^0)$, and denoting by $(x_1^t, \ldots, x_N^t)$ the set of particles obtained at step $t$, the scheme becomes
\begin{talign}
    \label{eq:discrete_opt_particles}
    x_{i}^{t+1}
    &= x_{i}^{t}
    +\frac{\epsilon}{N}\sum_{j=1}^{N} \big[ A_{t} A_{t}^\intercal s_p(x_j^t) k(A_{t}^\intercal x_{j}^{t},A_{t}^\intercal x_{i}^{t}) \nonumber \\
    &\quad + A_{t} \nabla_{x_1} k(A_{t}^\intercal x_{j}^{t},A_{t}^\intercal x_{i}^{t}) \big]
    ,\quad i=1,\ldots,N,\\
    \label{eq:discrete_opt}
    A_{t} &\in \arg\sup_{[A]\in\text{Gr}(d,m)}\alpha_t([A]),
\end{talign}
where $\alpha_t([A]) = \mbox{KSD}_{A}(Q_t, P)$, for $Q_t(dx) = \frac{1}{N}\sum_{i=1}^N \delta_{x_i^t}(dx)$. 


\begin{algorithm}[t!]
    \caption{Grassmann Stein Variational Gradient Descent (GSVGD)}
\label{alg:gsvgd}
\begin{algorithmic}[1]
\State {\bfseries Inputs:} $M$ initialized projectors $[A_{0, l}]\in\mbox{Gr}(d, m)$, $l = 1, \ldots, M$; $N$ initialised particles $\{x^{0}_{i}\}_{i=1}^N$; iteration number $n_\text{epochs}$; step sizes $\epsilon, \delta>0$.
\vspace{1mm}
\For{$t=1,2,\ldots,n_\text{epochs}$}
\State Update particles $x_{i}^{t+1}=x_{i}^{t}+\epsilon \sum_{l=1}^M \widehat{\phi}_{A_{t, l}}(x^t_i)$ for $i=1,\ldots,N$, where
\begin{talign}
    \widehat{\phi}_{A_{t, l}}(x^t_i) 
    &= \frac{1}{N}\sum_{j=1}^{N} \big[ \textcolor{red}{A_{t, l} A_{t, l}^\intercal} s_p(x_j^t) k(\textcolor{red}{A_{t, l}^\intercal} x_{j}^{t},\textcolor{red}{A_{t, l}^\intercal} x_{i}^{t}) \nonumber \\
    &\quad + \textcolor{red}{A_{t, l}} \nabla_{x_1} k(\textcolor{red}{A_{t, l}^\intercal} x_{j}^{t},\textcolor{red}{A_{t, l}^\intercal} x_{i}^{t}) \big].
    \label{eq: gsvgd update} 
\end{talign}
\State Update projectors
\begin{align*}
    A_{t+1, l}=\textrm{R}_{[A_{t, l}]}\left( \delta \Pi_{A_{t, l}} \nabla \alpha_t([A_{t, l}]) + \sqrt{2T \delta} \Pi_{A_{t, l}} \xi_{t, l}\right)
\end{align*}
for $l = 1, \ldots, M$, where $\xi_{t, l} \in \mathbb{R}^{d \times m}$ has i.i.d.\ $\mathcal{N}(0, 1)$ entries, and $\textrm{R}_{[A_{t, l}]}$ is defined in (\ref{eq: polar retr}). 
\EndFor
\State \textbf{Return:} Particles $\{x_{i}^{n_\text{epochs}}\}_{i=1}^N$.
    \end{algorithmic}
\end{algorithm}


\paragraph{Optimal Projections via SDEs:} Proposition~\ref{prop: optimal projection} implies the ``optimal'' projection $A_0$ is \emph{one} critical point of $\alpha_t$, but it does not imply the critical point is unique. Indeed, the problem (\ref{eq:sliced_objective_A}) is non-convex and there
might be multiple local maximisers, from which finding global maxima is generally NP-hard.  A well-known remedy is to add white noise to the gradient flow \citep{aluffi1985global,geman1986diffusions}, allowing the trajectory to escape from local maxima. Mathematically, such methods can be formulated in terms of Stochastic Differential Equations (SDEs).  In this particular instance, we explore the use of SDEs taking values on the Grassmann manifold. We consider stochastic dynamics defined by the solution of the following Stratonovich SDE
\begin{talign}
\label{eq:strat}
dA(t)
&= \mu \riemannGrad \alpha_t([A])\,dt + \sqrt{2T\mu} \Pi_{A_t}\circ dW(t),\\
&= \mu \Pi_{A(t)}\nabla \alpha_t([A(t)])\,dt + \sqrt{2T\mu} \Pi_{A(t)}\circ dW(t)\nonumber
\end{talign}
where $W(t)$ is a $\mathbb{R}^{d\times m}$-valued Brownian motion and $\mu, T > 0$. Combining the particle and projector evolution we can consider the full system as a discretisation of the following coupled ODE-SDE 
\begin{talign*}
    \dot{x}_i(t)  
    &=\frac{1}{N}A(t) \sum_{j=1}^{N} \big[
    \\ & A(t)^\intercal s_p(x_j(t)) k(A(t)^\intercal x_{j}(t),A(t)^\intercal x_{i}(t)) \\
    &+  \nabla_{x_2} k(A(t)^\intercal x_{j}(t),A(t)^\intercal x_{i}(t)) \big],\\
    dA(t)
    &= \mu \Pi_{A(t)}\nabla \alpha_t([A(t)])\,dt + \sqrt{2T\mu} \Pi_{A(t)}\circ dW(t).
\end{talign*}
We see that the parameter $T$ acts as a temperature, facilitating moving between local minima of the function $\alpha$ by annealing the loss function.  The parameter $\mu$ controls the relative timescale between the evolution of $A(t)$ and the particles $(x_1^t\ldots, x_N^t)$.  In particular, when $\mu \gg 1$, the distribution of $A(t)$ is approximated by the quasi-stationary distribution $d\mu_t([A])= e^{\alpha_t([A])/T}d[A]$, where $d[A]$ denotes the canonical measure on the Grassmann manifold.  In the other extreme, when $\mu \ll 1$  the projector $A(t)$ will evolve on a slower timescale than the particles, so that the particles will reach their stationary configuration for a fixed projector before it evolves.

To simulate the Stratonovich SDE \eqref{eq:strat}, we make use of the formulation of diffusions on a Riemannian manifold, making use of the associated retraction map, see \citet{staneva2017learning}, \citet{baxendale1976measures}, and \citet{belopolskaya2012stochastic} where the $\text{Gr}(d,m)$-valued SDE \eqref{eq:strat} can be expressed in the form of a system of Ito SDEs 
\begin{talign}
A(t) &= \textrm{R}_{[A(t)]}\left(B(t)\right),\\
\label{eq:tangent_sde}
dB(t) &=  \mu \Pi_{A(t)}\nabla \alpha_t([A(t)])\,dt + \sqrt{2T\mu}\Pi_{A(t)}dW_t.
\end{talign}
With step-size $\delta > 0$, an Euler-Maruyama discretisation for \eqref{eq:tangent_sde} results in
\begin{talign}
    A_{t+1} = \textrm{R}_{[A_t]}\left(\Pi_{A_t}\nabla \alpha_t([A_t])\,\delta + \sqrt{2T\delta}\Pi_{A_t}\xi_t\right),
    \label{eq: discretized projector update}
\end{talign}
where $\xi_t$ is a $d \times m$ matrix with independent Gaussian entries.  Note that we ``absorb'' the constant $\mu$ into the step-size $\delta$ for simplicity.

\paragraph{Batch Generalisation} 
An important observation is that at each step (\ref{eq:discrete_opt}), $x^{t+1}_i$ is different from $x^{t}_i$ only in the image of $A$. This contrasts with both SVGD as well as S-SVGD, both of which update the particles along all dimensions. One extension is to use more than one projector $A_{t, l} \in \bbR^{m_l \times d}$ for $l = 1, \ldots, M$, where $1 \leq M \leq d$ and $\sum_{l = 1}^M m_l \leq d$. At each optimisation step, we can impose orthonormality using QR factorisation, so that the $d \times d$ matrix $A_t$ formed by column-wise concatenation of $A_{t, 1}, \ldots, A_{t, M}$, is orthogonal. However, this requires $\calO(d^3)$ operations, which can be prohibitive for large $d$. We therefore propose to impose orthonormality every 1000 steps, which we find sufficient in practice. The full algorithm is presented in Algorithm \ref{alg:gsvgd}.

\paragraph{Computational Complexity}
Each iteration of the particles update in Algorithm~\ref{alg:gsvgd} requires $\calO(M N dm(N + d))$ operations. Compared with the $\calO(Nd (N + d))$ cost for S-SVGD, the extra factor $Mm$ arises from the fact that (\ref{eq: gsvgd update}) involves matrix multiplication with $A_{t, l}$, which can be avoided in S-SVGD due to simplification by using the canonical basis. However, this extra computation can be largely reduced by using a fixed number of projectors $M$ and projection dimension $m$. In our experiments, we find $M=20$ projectors are sufficient. A reasonable choice of $m$, however, will depend on the specific problem. Finally, each step of the projector update requires $\calO(M dm^2)$ due to the retraction map, which reduces to the same cost as the slice update in S-SVGD when $M = d$ and $m = 1$.



==> SteinsGate (final)/sections/5_related_work.tex <==
\paragraph{Connections to S-SVGD}
% Both our method and the S-SVGD of \citet{gong2021sliced} are based on KSD with a matrix-valued kernel, and both GKSD and the sliced kernel Stein Discrepancy (SKSD) require optimal projectors or slices in order to discriminate between two distributions. In a followup work, \citet{gong2021active} relaxed the optimality condition of the slices in SKSD, but they did not apply the new KSD variant to particle inference. 

The major differences between GSVGD and S-SVGD are that \emph{(i)} GSVGD allows projecting onto a arbitrary low-dimensional subspace, \emph{(ii)} GSVGD updates the projectors via Riemannian optimisation on the Grassmann manifold, whereas S-SVGD optimises the slices in the unit ball of $\bbR^d$, and \emph{(iii)} the projectors for the score function and the data are set to the same in GSVGD but not in S-SVGD. In particular, S-SVGD slices the score function with a fixed basis $O$ (i.e.\ the canonical basis), and such arbitrary choice may result in inefficient exploration of the state-space if the basis vectors $r \in O$ do not align with the latent dimensions of the target. On the other hand, optimising the projectors for the score function and the data separately would lead to a complex joint optimisation program that is practically challenging. GSVGD strikes a balance by using the same projector for the score function and the data.

\paragraph{Other SVGD Variants}
\citet{liu2018riemannian} extends SVGD to tasks defined on Riemannian manifolds and \cite{shi2021sampling} proposes a variant applied to non-Euclidean spaces (such as a simplex) via mirror descent. These are fundamentally different from our work, which concerns problems on the Euclidean space, while evolving the projectors on the Grassmann manifold. Closer to our method is the pSVGD of \citet{chen2020projected}, where the particles are projected onto a subspace defined by the top eigenvectors of a gradient information matrix. This method however suffers from practical issues, e.g.\ finding the eigen-decomposition would incur a computational cost that is cubic in the dimension. Other attempts to alleviate the curse-of-dimensionality problem of SVGD include Message Passing SVGD \citep{zhuo2018message} and graphical SVGD \citep{wang2018stein}, both of which are limited to problems where the target distribution is defined on a \emph{probabilistic graphical model} (PGM) with a known Markov structure. In contrast, GSVGD can be applied to distributions of an arbitrary form. 

% \citet{liu2018riemannian} extends SVGD to tasks defined on Riemannian manifolds and \cite{shi2021sampling} proposes a variant applied to non-Euclidean spaces (such as a simplex) via mirror descent. These are fundamentally different from our work, which concerns problems on the Euclidean space, while evolving the projectors on the Grassmann manifold. Closer to our method is the pSVGD of \citet{chen2020projected}, where the particles are projected onto a subspace defined by the top eigenvectors of a gradient information matrix. This method however suffers from some practical issues, e.g.\ finding the eigen-decomposition would incur a computational cost that is cubic in the dimension, and implementing this algorithm is non-trivial. For these reasons, we did not include pSVGD in our experiments. Other attempts to address the curse-of-dimensionality problem of SVGD include Message Passing SVGD \citep{zhuo2018message} and graphical SVGD \citep{wang2019stein}, both of which assume the target is defined on a \emph{probabilistic graphical model} (PGM) with a \emph{known} Markov structure, and hence are limited to such situations. In contrast, GSVGD can be applied to distributions of an arbitrary form. 
% 


==> SteinsGate (final)/sections/6_experiments.tex <==
We study the uncertainty quantification property of GSVGD against existing methods such as SVGD and S-SVGD on a number of experiments. We conclude from our experiments that SVGD can underestimate the uncertainty, S-SVGD can overestimate it and GSVGD, with appropriate projection dimensions, yields the best estimates. For GSVGD, we use the batch approach of Algorithm~\ref{alg:gsvgd}, where at most $M=20$ projectors with the same projection dimension $m$ are used. The temperature $T$ is set to a small value and is gradually incremented to a larger one via an annealing scheme. The learning rates for all methods are tuned for optimal performance on the multimodal mixture example, and the same choices are used for the other experiments.

In all experiments, we use the Gaussian RBF kernel parameterised by $k(x, x^\prime) = \exp\left(  -\| x - x^\prime \|_2^2/(2\sigma^2)\right)$ with bandwidth $\sigma^2 = \texttt{med}^2 / (2 \log n)$, where $\texttt{med}$ is the median of the pairwise distance of the particles. This follows the heuristic in \citet{Liu2016SVGD}. To quantify sample quality, we use the \emph{energy distance} \citep{szekely2013energy} between the approximation and the ground truth. However, we find that the energy distance is not sensitive to differences in correlations between multivariate samples. Therefore, we also evaluate how well each method captures the dependence between multivariate samples by the covariance estimation error $||\hat{\Sigma} - \Sigma||_{2}$, where $||\cdot||_2$ is the Frobenius norm, $\Sigma$ is the ground truth sample covariance matrix given by a Hamiltonian Monte Carlo (HMC) (for non-synthetic data), and $\hat{\Sigma}$ is the estimated covariance. For further details, see Appendix~\ref{appendix: experimental details}. All the code is available at \url{https://github.com/ImperialCollegeLondon/GSVGD}.

\begin{figure}
    % \vspace{-3mm}
    \centering
    \includegraphics[width=0.23\textwidth]{figs/gaussian/var.pdf}
    \vspace{-3mm}
    \caption{Estimating the dimension-averaged marginal variance of $p(x) = \calN(x; 0, I_d)$ across different dimensions $d$. GSVGD1 means GSVGD with 1-dimensional projections. Black solid line marks the true value. Results are averaged over 20 repetitions.}
    \label{fig: gaussian marginal var}
    % \vspace{-5mm}
\end{figure}

\paragraph{Multivariate Gaussian}
The first toy example is a $d$-dimensional multivariate Gaussian $p(x) = \calN(x; 0, I_d)$. For each method, 500 particles are initialized from $\calN(x; 2 \mathds{1}, 2I_d)$, where $\mathds{1} \in \bbR^d$ denotes the vector of ones. This is a standard benchmark used to illustrate the diminishing variance issue of SVGD \citep{Liu2016SVGD, gong2021sliced, zhuo2018message}. We show empirically that GSVGD is able to mitigate this problem by plotting the dimension-averaged estimates for the marginal variance in Figure~\ref{fig: gaussian marginal var}. We see that GSVGD estimates stay roughly at 1 for all dimensions as expected, whereas the SVGD estimates scale inversely with dimension. S-SVGD, on the other hand, over-estimates the variance. We remark, however, that GSVGD5 appears to be biased with a lower variance. This is due to the variance underestimation issue of SVGD persisting in 5 dimensional subspaces. 


\paragraph{Multimodal Mixture}
In the second example, the target distribution is a mixture of $4$ $d$-dimensional Gaussian distributions $p(x) = \sum_{k = 1}^{4} 0.25 \mathcal{N}(x; \mu_k, I_d)$ with uniform mixture ratios. The first two coordinates of the mean vectors are equally spaced on a circle, while the other coordinates are set to 0; see Figure~\ref{fig: multimodal particles 50d} and Appendix~\ref{appendix:multimodal}. Particles are initialized from $\calN(0, I_d)$ and only the first two dimensions need to be learned. The primary goal is to investigate whether GSVGD can efficiently recover this low-dimensional latent structure by adapting the projectors. As shown in \ref{fig: multimodal energy}, GSVGD1 and GSVGD2 outperforms S-SVGD in all dimensions in terms of the energy distance, while GSVGD5 is able to achieve a competitive performance. SVGD, on the other hand, fails to capture the uncertainty of the target, as shown in Figure~\ref{fig: multimodal particles 50d}. 

% That is, the first two coordinates are equally spaced on a circle of radius $\sqrt{5}$ in $\bbR^2$, while the others are centred at the origin 
\begin{figure}[t!]
    \centering
    % \vspace{-6mm}
    \subfigure[Multimodal mixture]
    {
        \label{fig: multimodal particles 50d}
        \includegraphics[width=0.22\textwidth]{figs/multimodal/final_particles_50d.png}
    }
    \subfigure[X-shaped mixture]
    {
        \label{fig: xshaped particles 50d}
        \includegraphics[width=0.22\textwidth]{figs/xshaped/final_particles_50d.png}
    }
    \vspace{-4mm}
    \caption{Marginals of target and estimated densities in the first 2 dimensions. Red dots are the particles after 2000 iterations and the target density is shown by the contour. Both targets have dimension 50.}
    \label{fig: final particles}
\end{figure}

\begin{figure}[t!]
    \centering
    % \vspace{-6mm}
    \subfigure[Multimodal mixture]
    {
        \label{fig: multimodal energy}
        \includegraphics[width=0.22\textwidth]{figs/multimodal/energy.pdf}
    }
    \subfigure[X-shaped mixture]
    {
        \label{fig: xshaped energy}
        \includegraphics[width=0.22\textwidth]{figs/xshaped/energy.pdf}    
    }
    % \subfigure[X-shaped mixture convergence \xl{move to appendix?}]
    % {
    %     \label{fig: xshaped energy vs epochs}
    %     \includegraphics[width=0.26\textwidth]{figs/xshaped/energy_50d.pdf}
    % }
    \vspace{-4mm}

    \caption{Energy distance between the target distribution and the particle estimation. Results are averaged over 20 repetitions. $95\%$-confidence intervals are shown by the shaded regions.}
    % (c): Energy distance against iterations in the 50-dimensional X-shaped example.}
    \label{fig: summary metrics}
    % \vspace{-5mm}
\end{figure}


\paragraph{X-Shaped Mixture}
The target in this experiment is a $d$-dimensional mixture of two correlated Gaussian distributions $p(x) = 0.5 \mathcal{N}(x; \mu_1, \Sigma_1) + 0.5 \mathcal{N}(x; \mu_2, \Sigma_2)$. The means $\mu_1, \mu_2$ of each Gaussian have components equal to 1 in the first two coordinates and 0 otherwise, and the covariance matrices admit a correlated block diagonal structure (see Appendix~\ref{appendix:xshaped}). The mixture hence manifests as an ``X-shaped'' density marginally in the first two dimensions (see Figure~\ref{fig: xshaped particles 50d}). Figure~\ref{fig: xshaped energy} shows that GSVGD1 and GSVGD2 achieve a better approximation quality than both SVGD and S-SVGD across all dimensions. This is further verified by plotting the first two coordinates of the final particles in \ref{fig: final particles} (b). On the other hand, GSVGD5 shows a slightly suboptimal performance for dimensions larger than 30. This is potentially because of the inefficiency due to projecting the particles to 5 dimensional subspace in the case we only care about the first 2.

\paragraph{Conditioned Diffusion Process}

\begin{figure}[t!]
    \centering
    % \vspace{-5mm}
    \includegraphics[width=0.48\textwidth]{figs/diffusion/solution.pdf}
    \vspace{-8mm}
    \caption{HMC, SVGD, S-SVGD and GSVGD solutions, as well as the posterior mean and $95\%$ confidence interval after 1000 iterations. }
    \label{fig: diffusion solution}
    % \vspace{-4mm}
\end{figure}

The next example is a benchmark that is often used to test inference methods in high dimensions \citep{cui2016dimension, chen2020projected, detommaso2018stein}. We consider a stochastic process $u: [0, 1] \to \bbR$ governed by
\begin{talign}
    du_t = \frac{10u(1 - u^2)}{1 + u^2} dt + dx_t, 
    \quad
    u_t = 0,
    \label{eq: diffusion process}
\end{talign}
where $t \in (0, 1]$, and the forcing term $x = (x_t)_{t \geq 0}$ follows a Brownian motion so that $x \sim q = \calN(0, C)$ with $C(t, t') = \min(t, t')$. We observe noisy data $y = (y_{t_1}, \ldots, y_{t_{20}})^\intercal \in \bbR^{20}$ at 20 equi-spaced time points $t_i = 0.05i$, where $y_{t_i} = u_{t_i} + \epsilon$ for $\epsilon \sim \calN(0, \sigma^ 2)$ with $\sigma = 0.1$, and $u_{t_i}$ is generated by solving (\ref{eq: diffusion process}) at a true Brownian path $x_{\textrm{true}}$. The goal is to use $y$ to infer the forcing term $x$ and thereby the solution state $u$. 

The prior we use for $x$ is the Brownian motion described above. The dynamic is discretized using an Euler-Maruyama scheme with step size $\Delta t = 10^ {-2}$, leading to a 100-dimensional inference problem. Due to the smoothness of the Brownian path, we expect the solution $u$ to have an intrinsic low-dimensional structure. Figure~\ref{fig: diffusion solution} shows the mean and 95$\%$ credible intervals of the particle estimation of $u$ after 1000 iterations. Compared with a reference HMC, all methods are able to estimate the mean accurately, but SVGD and S-SVGD either underestimate or overestimate the credible intervals. GSVGD projecting on $20$ dimensions gives the most accurate uncertainty estimates. Choosing a good projection dimension is non-trivial even in this simple problem; however, by plotting the energy distance between the HMC reference and the results against different projection dimensions (Figure \ref{fig: diffusion energy} of Appendix), we see that so long as we do not project onto very low or high dimensions, GSVGD achieves a greater degree of agreement with the reference HMC than SVGD and S-SVGD. 

\paragraph{Bayesian Logistic Regression} 
Following \cite{Liu2016SVGD}, we consider the Bayesian logistic regression model applied to the Covertype dataset \citep{asuncion2007uci}. We use HMC posterior samples as a gold standard for evaluating the posterior approximations. We ran all methods on a subset consisting 1,000 randomly selected data points 10 times. Similar to the synthetic experiments, we see in Figure~\ref{fig:blr:covariance_estimation} that there exists an optimal projection dimension (around $m=10$) such that GSVGD more accurate approximates the covariance matrix whilst yielding similar energy distances as S-SVGD. S-SVGD severely overestimates the uncertainty, also shown in Figure~\ref{fig:blr:cov.pdf}, whereas SVGD severely underestimates it.

\begin{figure}[t!]
\centering
% \vspace{-5mm}
\subfigure[Energy distance against projection dimensions]{
\includegraphics[width=0.22\textwidth]{figs/blr/EnergyDistance.pdf}
}
\label{fig:blr:energy distance}
\subfigure[$||\hat{\Sigma}-\Sigma||_2$ against projection dimensions]{
\includegraphics[width=0.22\textwidth]{figs/blr/CovarianceError.pdf}
}
\vspace{-3mm}
\caption{Metrics for Covertype.}
\label{fig:blr:covariance_estimation}
\end{figure}


==> SteinsGate (final)/sections/7_conclusion.tex <==
We introduced Grassmann Stein Variational Gradient Descent (GSVGD), a novel extension to the SVGD algorithm, to tackle the curse-of-dimensioanlity problem. At each step, GSVGD seeks the subspace in which the proposal and the target has the largest discrepancy measured by the Grassmann Kernel Stein Discrepancy (GKSD). The evolution of the particles and the projector is determined through a coupled ODE-SDE system, which allows trade-offs between exploration and exploitation. The GSVGD algorithm can be easily extended to a batched version that uses more than one projector. Our experiments demonstrate that GSVGD is able to achieve improved performance over existing methods when the target distribution has an intrinsic low-dimensional structure, especially more accurately quantifying the epistemic uncertainty.

\paragraph{Limitations of GSVGD:} One limitation of GSVGD is the choice of projection dimension and number of projectors to use in order to attain superior performance. One possible way is to perform a grid search over a range of feasible values and then assess the performance using metrics that measure particle diversity. We leave this as an open question for future work. In addition, our Grassmann-valued SDE introduces additional hyperparameters, which potentially require tuning on a case-by-case basis for each problem. In Section~\ref{sec: experiments} we present some heuristics for tuning GSVGD hyperparameters that we found yielded consistent results, but we would recommend future work to study the sensitivity of the hyperparameters.
% Possible future works include a theoretical study on the convergence of the coupled particle-projector evolution...



% Possible future works include theoretical studies on the dynamic of the particles-projector evolution, as well as robustness analyses with respect to different choices of hyper-parameters (learning rates for the particles and projectors; temperature $T$). Furthermore, applying the discrepancy GKSD to tasks such as goodness-of-fitting tests \citep{Liu2016, gretton2012kernel, jitkrittum2017linear} or model learning \citep{grathwohl2020cutting, feng2017learning, pu2017vae} is also an interesting direction.

\begin{figure}[t!]
\centering
% \vspace{-4mm}
\includegraphics[width=0.45\textwidth]{figs/blr/cov.pdf}
\vspace{-3mm}
\caption{Covariance matrices for Covertype.}
% \vspace{-5mm}
\label{fig:blr:cov.pdf}
\end{figure}
